From Internal Diagnosis to External Auditing: A VLM-Driven Paradigm for Data-Free Online Backdoor Defense

Deep Neural Networks remain inherently vulnerable to backdoor attacks. Traditional test-time defenses largely operate under the paradigm of internal diagnosis methods like model repairing or input robustness, yet these approaches are often fragile under advanced attacks as they remain entangled with the victim model's corrupted parameters. We propose a paradigm shift from Internal Diagnosis to External Semantic Auditing, arguing that effective defense requires decoupling safety from the victim model via an independent, semantically grounded auditor. To this end, we present a framework harnessing Universal Vision-Language Models (VLMs) as evolving semantic gatekeepers. We introduce PRISM (Prototype Refinement & Inspection via Statistical Monitoring), which overcomes the domain gap of general VLMs through two key mechanisms: a Hybrid VLM Teacher that dynamically refines visual prototypes online, and an Adaptive Router powered by statistical margin monitoring to calibrate gating thresholds in real-time. Extensive evaluation across 17 datasets and 11 attack types demonstrates that PRISM achieves state-of-the-art performance, suppressing Attack Success Rate to <1% on CIFAR-10 while improving clean accuracy, establishing a new standard for model-agnostic, externalized security.

==> section_11_ethnical.tex <==
% \clearpage
% \section{Ethical Considerations}

% In this research, we evaluated \system{} and demonstrated its high Attack Success Rate (ASR) across various scenarios, including prominent real-world APIs such as Google, Baidu, Taobao, and JD. 

% During our attack evaluation, we adhered to best practices to ensure safety and minimize any potential harm arising from our research. We only steer the victim systems (or models) to generate misclassification results for those inputs where incorrect predictions would not lead to financial loss or the exposure of inappropriate content. We also responsibly disclosed our findings to the organizations managing the image search services and Large Language Models (LLMs) analyzed in our study.


% From the defender's perspective, we studied the potential mitigation to our attack. In Section~\ref{sec:defenses}, we evaluated the effectiveness of both existing and adaptive defenses against our newly proposed attack. Our analysis revealed that adversarial training (discussed in Section~\ref{sec:adversarial_training}) can lower the ASR of our attack, though this comes at the cost of reduced accuracy on benign inputs.

% The societal benefits of our research outweigh the potential harm. First, we uncovered a new risk in which adversaries could exploit open-source vision-language models to manipulate the outputs of victim models. We demonstrated that this threat is real to popular image-search APIs. This early warning is valuable for companies managing these APIs, aiding in risk control and potentially mitigating future losses. 
% Second, our work introduces a more realistic threat model for examining backdoor or adversarial example attacks on DNN models, where access to both the model and dataset is limited. Under this threat model, we demonstrated that attacks can still succeed, and conducted an initial study on defense strategies, moving a step closer to practical solutions.
% Third, we offered insights on how to tailor general vision-language models for specific tasks (mimicking the target model in our scenario), providing useful guidance for future researchers.


% \section{Open Science}

% In the spirit of open science, we have made our codebase publicly available on Anonymous GitHub. This repository includes a comprehensive training and evaluation toolkit, pre-trained models under various norms tailored for different target datasets, and samples of perturbed images as discussed in our case studies. Access to these resources can be found at the following link: \url{https://anonymous.4open.science/r/UnivIntruder}. Upon acceptance of our work, the repository will be transferred to a public GitHub repository.

==> section_4_methodology_old.tex <==

\vspace{-8pt}
\section{Methodology}
\vspace{-5pt}

\subsection{Overview of PRISM}
\vspace{-5pt}
To secure deployed models against diverse backdoor attacks without accessing training data, we propose \textbf{PRISM} (\textbf{P}rototype \textbf{R}efinement \& \textbf{I}nference via \textbf{S}tatistical \textbf{M}argin). As illustrated in Fig. \ref{fig:pipeline}, PRISM functions as a test-time wrapper around the suspicious victim model. The core intuition is that while backdoor triggers force the victim model to output high-confidence predictions on poisoned samples, these predictions often lack semantic support in the feature space of a benign, general-purpose Vision-Language Model (VLM). PRISM exploits this semantic discrepancy through a three-pillar architecture: (1) A \textbf{Dual Stream Inference} framework that processes inputs through both the victim model and a trusted Universal VLM Teacher; (2) A \textbf{Hybrid VLM Teacher} that enhances zero-shot capabilities by fusing static text anchors with dynamically refined visual prototypes; and (3) An \textbf{Adaptive Router} that employs online statistical monitoring to gate predictions based on a difficulty-aware logit margin. By continuously updating the statistical moments and visual prototypes using only high-confidence clean samples, PRISM adapts to the test stream distribution in an online manner, effectively filtering out backdoor triggers while preserving benign performance.

\vspace{-8pt}
\subsection{Dual Stream Inference Framework}
\vspace{-5pt}
The foundation of PRISM is a parallel inference mechanism designed to decouple the potential risk from the decision process. For any incoming test sample \( x \), the system initiates two concurrent forward passes. The first stream passes \( x \) through the suspicious model \( f_S \), yielding a prediction \( \hat{y}_S \) and its associated logits. While \( f_S \) is potentially compromised, it typically possesses high domain-specific utility. The second stream processes \( x \) through a frozen, trusted VLM backbone. Unlike prior works that rely solely on static zero-shot classification, which may suffer from domain shifts, our framework treats the VLM as a "Universal Teacher" that provides a semantic verification signal. The outputs of these two streams—the suspicious logits from the victim and the robust logits from the hybrid VLM—are then fed into the Adaptive Router. This dual-stream design ensures that the system defaults to the high-performance victim model for benign samples but falls back to the robust VLM prediction when a backdoor attack is detected, creating a fail-safe mechanism that balances utility and security.

\vspace{-5pt}
\subsection{Universal Hybrid VLM Teacher}
\vspace{-5pt}
A critical limitation of using standard VLMs for defense is their variable zero-shot performance on specialized downstream tasks. To address this, we introduce a Universal VLM Backbone that supports both embedding-based models (e.g., CLIP, SigLIP) and generative models (e.g., Qwen, Gemma), enhanced by a hybrid anchoring mechanism.

\textbf{Universal Backbone Support.}
For embedding-based VLMs, we compute the cosine similarity between the image embedding \( z_{img} \) and the text embeddings \( z_{text} \) of the candidate class labels. For generative VLMs, which are typically computationally intensive, we optimize inference using a Key-Value (KV) Cache strategy. We construct a prompt template \( Q \): "Classify this image", and evaluate the probability of the model generating specific class names as answers (e.g., \( A \): "It is \{candidate\}"). By caching the visual features and the system prompt's hidden states, we avoid redundant computations for the invariant parts of the input. The classification logits are derived from the language modeling loss associated with each candidate label token, effectively converting the generative output into a discriminative probability distribution.

\textbf{Hybrid Anchors: Text and Prototypes.}
To further robustify the VLM's judgment, we employ a hybrid fusion strategy. While text anchors (from prompt templates like "A photo of a \{class\}") provide general semantic guidance, they may fail to capture fine-grained intra-class variance. We therefore augment the VLM with Visual Prototypes (Class Centroids), denoted as \( \mathcal{C} = \{c_1, \ldots, c_K\} \). These prototypes are initialized (or empty-initialized) and dynamically refined during inference. The final VLM logits \( S_{VLM} \) are computed via weighted fusion of text-image similarity logits \( S_{text} \) and image-prototype similarity logits \( S_{proto} \):
\vspace{-6pt}
\[
S_{VLM} = \lambda \cdot S_{proto} + (1 - \lambda) \cdot S_{text},
\]
where \( \lambda \) is a balancing coefficient. This hybrid approach allows the VLM teacher to use both the broad semantic knowledge of language and the specific visual distribution of the current test stream.

\vspace{-8pt}
\subsection{Adaptive Router via Statistical Monitoring}
\vspace{-5pt}
The core decision logic of PRISM resides in the Adaptive Router, which determines whether to accept the victim model's prediction or reject it in favor of the VLM. This decision is governed by a statistical discrepancy test based on the Logit Margin.

\textbf{Logit Margin Calculation.}
We define a discrepancy metric $\Delta$ that quantifies the semantic support the VLM provides for the victim model's prediction. Let $\hat{y}_S$ be the class predicted by the suspicious model. We examine the VLM's logits $S_{VLM}$ specifically at the index $\hat{y}_S$ and compare it to the maximal logit of all other classes $i \neq \hat{y}_S$. The logit margin $\Delta$ is formally defined as:
\vspace{-6pt}
\[
\mathrm{\Delta}=\exp{\left(S_{VLM}^{\hat{y}_S}-\max\limits_{i \neq \hat{y}_S}{S_{VLM}^i}\right)}
\]
We employ the exponential transformation to ensure \textbf{statistical stability}. Since raw logit differences are unbounded and can approach $-\infty$ when the VLM strongly rejects the victim's prediction, the exponential mapping suppresses these extreme negative outliers, confining the metric to a robust positive range. Consequently, a small $\Delta$ (near 0) implies strong disagreement, while a large $\Delta$ indicates alignment. In backdoor scenarios, the victim model is overconfident on the target class due to the trigger, while the VLM, being blind to the trigger, predicts the ground truth class, leading to a significant discrepancy and a sharp drop in $\Delta$.

\textbf{Adaptive Thresholding via Cornish-Fisher Expansion.}
A static threshold for \( \Delta \) is insufficient due to the varying difficulty of classes and the non-Gaussian, often skewed nature of the discrepancy distribution. To address this, we model the distribution of \( \Delta \) for each class \( k \) in an online manner. We maintain the running statistics of \( \Delta \), specifically the mean \( \mu_k \), standard deviation \( \sigma_k \), and skewness \( \gamma_{k} \) (the third standardized moment). 

We employ the Cornish-Fisher expansion to derive an adaptive threshold \( \tau_k \). This method approximates the quantiles of a non-Gaussian distribution by correcting the standard normal quantile based on higher-order moments. Let \( \zeta \) denote the \textit{base confidence coefficient} (a hyperparameter corresponding to the target Z-score in a standard normal distribution, e.g., \( \zeta=-2 \) targets a \( \approx 97.7\% \) clean acceptance rate). The skewness-adjusted effective coefficient \( \tilde{\zeta}_k \) is calculated as:
\vspace{-6pt}
\[
\tilde{\zeta}_k = \zeta + \frac{\gamma_{k}}{6}(\zeta^2 - 1).
\]
This correction term shifts the threshold to account for the asymmetry of the margin distribution. Specifically, positive skewness (long tail to the right) raises the threshold to reduce false rejections, while negative skewness lowers it. The final adaptive threshold for class \( k \) is then defined as:
\vspace{-6pt}
\[
\tau_k = \mu_k + \tilde{\zeta}_k \cdot \sigma_k.
\]
To ensure stability during the cold-start phase, we further apply a time-dependent confidence weight \( w_t \) to the correction term, which gradually activates the skewness adjustment as more images are observed. If the discrepancy \( \Delta \) of a test sample exceeds \( \tau_k \), it is deemed consistent and accepted; otherwise, it is flagged as a potential attack.

\begin{table*}
\caption{\textbf{Comparative evaluation of backdoor defenses on CIFAR-10.} ASRs below 15\% are highlighted in \smash{\colorbox{customblue}{blue}} (success), while those above 15\% are in \smash{\colorbox{customred}{red}} (failure). \system{} is the only method that successfully defends against all 11 attack types while maintaining high Clean Accuracy (CA), whereas existing SOTA defenses fail significantly on Clean-Image backdoors (FLIP, GCB) or Dynamic attacks.}
\label{tab:cifar10_compare}
\vspace{-0.15cm}
\centering
\resizebox{\linewidth}{!}{
\begin{small}
\begin{tblr}{
  width = 1.0\linewidth,
  rowsep = 0.8pt,
  colsep = 1.55pt,
  cells = {c},
  cell{1}{1} = {c=2,r=2}{},
  cell{1}{3} = {c=2,r=2}{},
  cell{1}{5} = {c=14}{},
  cell{1}{19} = {c=4}{},
  cell{1}{23} = {c=2,r=2}{},
  cell{2}{5} = {c=2}{},
  cell{2}{7} = {c=2}{},
  cell{2}{9} = {c=2}{},
  cell{2}{11} = {c=2}{},
  cell{2}{13} = {c=2}{},
  cell{2}{15} = {c=2}{},
  cell{2}{17} = {c=2}{},
  cell{2}{19} = {c=2}{},
  cell{2}{21} = {c=2}{},
  cell{3}{1} = {c=2}{},
  cell{4}{1} = {r=2}{},
  cell{6}{1} = {r=4}{},
  cell{10}{1} = {r=3}{},
  cell{13}{1} = {r=2}{},
  cell{15}{1} = {c=2}{},
  cell{16}{1} = {c=4}{},
  cell{17}{1} = {c=4}{},
  hline{1,18} = {-}{0.1em},
  hline{2} = {5,19}{l},
  hline{2} = {18,22}{r},
  hline{2} = {6-17}{},
  hline{2} = {20-21}{},
  hline{3} = {3,5,7,9,11,13,15,17,19,21,23}{l},
  hline{3} = {4,6,8,10,12,14,16,18,20,22,24}{r},
  hline{4,6,10,13,15-16} = {-}{0.05em},cell{4}{4,12,22} = {bg = customred},
  cell{4}{6,8,10,14,16,18,20,24} = {bg = customblue},
  % Blend (Row 5)
  cell{5}{4,6,8,14,16,22} = {bg = customred},
  cell{5}{10,12,18,20,24} = {bg = customblue},
  % WaNet (Row 6)
  cell{6}{4,8,10,12,14,16,22} = {bg = customred},
  cell{6}{6,18,20,24} = {bg = customblue},
  % BPP (Row 7)
  cell{7}{4,14,22} = {bg = customred},
  cell{7}{6,8,10,12,16,18,20,24} = {bg = customblue},
  % IAB (Row 8)
  cell{8}{4,10,14,22} = {bg = customred},
  cell{8}{6,8,12,16,18,20,24} = {bg = customblue}, % Ensemble(22) is 17.9
  % SSBA (Row 9)
  cell{9}{4,6,16,22} = {bg = customred},
  cell{9}{8,10,12,14,18,20,24} = {bg = customblue},
  % CTRL (Row 10)
  cell{10}{4,8,14,16,22} = {bg = customred},
  cell{10}{6,10,12,18,20,24} = {bg = customblue},
  % SIG (Row 11)
  cell{11}{4,6,8,10,16,14,22} = {bg = customred},
  cell{11}{12,18,20,24} = {bg = customblue},
  % LC (Row 12)
  cell{12}{4,6,14,22} = {bg = customred},
  cell{12}{8,12,10,16,18,20,24} = {bg = customblue}, % CLP(6) is 18.4
  % FLIP (Row 13)
  cell{13}{4,6,10,12,14,18,22} = {bg = customred},
  cell{13}{8,16,20,24} = {bg = customblue},
  % GCB (Row 14)
  cell{14}{4,6,8,10,12,14,16,18,22} = {bg = customred},
  cell{14}{20,24} = {bg = customblue},
  % Average (Row 15)
  cell{15}{4,6,8,10,12,16,14,22} = {bg = customred},
  cell{15}{18,20,24} = {bg = customblue},
}
Defense →                   &        & No Defense &      & Existing Backdoor Defenses &      &         &      &      &      &      &      &      &      &      &      &        &      & Naive VLM Baselines &      &          &      & {PRISM \\ (Ours)} &      \\
                            &        &            &      & CLP                        &      & ScaleUp &      & ZIP  &      & TeCo &      & C\&C   &      & LPP  &      & Refine &      & Zero-shot           &      & Ensemble &      &          &      \\
Attack ↓                    &        & CA         & ASR  & CA                         & ASR  & CA      & ASR  & CA   & ASR  & CA   & ASR  & CA   & ASR  & CA   & ASR  & CA     & ASR  & CA                  & ASR  & CA       & ASR  & CA       & ASR  \\
{Classic \\Backdoor}        & BadNet & 92.3       & 87.9 & 90.7                       & 12.4 & 90.2    & 0.2  & 86.4 & 9.1  & 92.4 & 26.4 & 90.3 & 9.5  & 90.7 & 3.3  & 90.7   & 1.7  & 86.7                & 0.2  & 94.9     & 50.4 & 93.9     & 0.0  \\
                            & Blend  & 93.6       & 99.4 & 90.3                       & 76.3 & 84.1    & 97.5 & 87.3 & 5.7  & 83.8 & 0.8  & 84.7 & 50.7 & 83.9 & 15.9 & 91.6   & 2.9  & 86.7                & 0.2  & 95.5     & 95.3 & 94.2     & 0.0  \\
{Dynamic \\Backdoor}        & WaNet  & 91.1       & 94.1 & 89.1                       & 2.0  & 76.2    & 89.2 & 45.6 & 70.9 & 92.0 & 99.0 & 91.1 & 94.0 & 89.0 & 43.3 & 82.9   & 2.2  & 86.7                & 0.3  & 95.0     & 59.8 & 93.6     & 0.0  \\
                            & BPP    & 91.5       & 99.4 & 91.2                       & 1.7  & 85.3    & 0.4  & 83.8 & 2.2  & 88.7 & 10.9 & 90.4 & 86.1 & 91.3 & 1.9  & 90.3   & 1.1  & 86.7                & 0.4  & 94.6     & 95.2 & 93.7     & 1.1  \\
                            & IAB    & 91.5       & 95.0 & 91.1                       & 4.5  & 82.9    & 2.3  & 82.3 & 61.3 & 80.8 & 7.9  & 86.0 & 25.4 & 90.5 & 2.9  & 91.1   & 6.0  & 86.7                & 0.5  & 94.4     & 17.9 & 92.4     & 0.0  \\
                            & SSBA   & 93.0       & 97.3 & 90.7                       & 42.8 & 83.7    & 0.0  & 88.1 & 10.4 & 84.3 & 4.5  & 84.0 & 13.0 & 90.5 & 29.4 & 60.9   & 5.9  & 86.7                & 0.3  & 95.1     & 88.0 & 93.8     & 0.0  \\
{Clean-Label \\Backdoor}    & CTRL   & 93.6       & 95.9 & 91.7                       & 0.9  & 82.4    & 43.1 & 88.3 & 1.6  & 85.3 & 11.8 & 93.1 & 95.3 & 92.7 & 36.1 & 91.1   & 4.8  & 86.7                & 0.4  & 95.7     & 75.7 & 94.2     & 0.0  \\
                            & SIG    & 93.6       & 93.9 & 90.3                       & 93.5 & 84.5    & 79.3 & 90.0 & 97.3 & 83.5 & 6.2  & 85.7 & 34.6 & 92.4 & 93.2 & 90.5   & 0.3  & 86.7                & 0.7  & 95.4     & 80.7 & 92.6     & 2.2  \\
                            & LC     & 93.4       & 98.4 & 87.4                       & 18.4 & 88.2    & 0.0  & 89.7 & 1.0  & 84.2 & 7.2  & 85.4 & 30.9 & 89.4 & 12.2 & 91.5   & 2.0  & 86.7                & 0.3  & 95.5     & 73.5 & 94.6     & 0.0  \\
{Clean-Image \\Backdoor}    & FLIP   & 89.9       & 99.2 & 89.1                       & 28.5 & 81.5    & 0.1  & 86.5 & 87.6 & 85.3 & 50.0 & 87.3 & 69.1 & 82.2 & 9.6  & 88.8   & 30.3 & 86.7                & 0.2  & 93.8     & 96.3 & 91.7     & 1.1  \\
                            & GCB    & 88.6       & 100. & 89.1                       & 100. & 81.5    & 100. & 78.7 & 100. & 88.9 & 100. & 86.9 & 100. & 90.2 & 69.4 & 86.4   & 100. & 86.7                & 0.4  & 92.3     & 100. & 90.1     & 4.4  \\
Average                     &        & 92.0       & 96.4 & 90.1                       & 34.6 & 83.7    & 37.5 & 82.4 & 40.6 & 86.3 & 29.5 & 87.7 & 55.3 & 89.3 & 28.8 & 86.9   & 14.3 & 86.7                & 0.4  & 94.7     & 75.7 & 93.2     & 0.8  \\
CA Drop (smaller is better) & & & & \drop{1.9} & & \drop{8.3} & & \drop{9.6} & & \drop{5.7} & & \drop{4.3} & & \drop{2.7} & & \drop{5.1} & & \drop{5.3} & & \rise{2.7} & & \rise{1.2} & \\
ASR Drop (larger is better) & & & & & \drop{61.8} & & \drop{58.9} & & \drop{55.8} & & \drop{66.9} & & \drop{41.1} & & \drop{67.6} & & \drop{82.1} & & \drop{96.0} & & \drop{20.7} & & \drop{95.6}
\end{tblr}
\end{small}
}
\vspace{-0.5cm}
\end{table*}

\vspace{-8pt}
\subsection{Online Update and Prototype Refinement}
\vspace{-5pt}

PRISM uses a self-evolving mechanism to adapt to the test-time distribution. To avoid cold-start instability (e.g., immediate attack flooding), we introduce a safe warm-up protocol. We assume a brief initialization window of the first $N$ samples where the stream is benign-dominant. During warm-up, PRISM relies on static text-based gating to filter obvious outliers while aggressively aggregating high-confidence samples to initialize visual prototypes and statistical moments ($\mu, \sigma, \gamma$). After establishing a statistical baseline ($t > N$), the system switches to full adaptive routing. Post warm-up, we apply a strict feedback loop that updates internal states only when a sample is certified as clean (i.e., $\Delta > \tau$). This continuous refinement progressively aligns the Hybrid VLM Teacher with the target domain while preventing poisoned updates from rejected attack samples.
